Computing Adequately Permissive Assumptions for Synthesis

We solve the problem of automatically computing a new class of environment assumptions in two-player turn-based finite graph games which characterize an ``adequate cooperation'' needed from the environment to allow the system player to win. Given an $\omega$-regular winning condition $\Phi$ for the system player, we compute an $\omega$-regular assumption $\Psi$ for the environment player, such that (i) every environment strategy compliant with $\Psi$ allows the system to fulfill $\Phi$ (sufficiency), (ii) $\Psi$ can be fulfilled by the environment for every strategy of the system (implementability), and (iii) $\Psi$ does not prevent any cooperative strategy choice (permissiveness). For parity games, which are canonical representations of $\omega$-regular games, we present a polynomial-time algorithm for the symbolic computation of adequately permissive assumptions and show that our algorithm runs faster and produces better assumptions than existing approaches -- both theoretically and empirically. To the best of our knowledge, for $\omega$-regular games, we provide the first algorithm to compute sufficient and implementable environment assumptions that are also permissive.

==> sections/motivating_example.tex <==
% !TEX root=main.tex

\subsection{Motivating example}
\label{sec:motivating example}

We use the simple two-player games in Fig.~\ref{fig:illustration of assumptions} to illustrate the main idea of \aname assumptions.
%; all the assumptions that will be discussed are sufficient and implementable, which are standard notions and will be discussed in Sec.~\ref{section:maximally permissive assumptions}.
From now on, we call the system player '$\pz$' and the environment player '$\po$'.
In Fig.~\ref{fig:illustration of assumptions}, we demonstrate four games played on four different \emph{game graphs}, which are finite directed graphs whose set of vertices are partitioned into $\pz$ and $\po$ vertices, shown using circles and squares, respectively.
The game starts by placing a token in one of the vertices, and at every time step, if the token is in a $\p{i}$ vertex $v$ then $\p{i}$ moves it to one of the successors of $v$.
A \emph{strategy} of $\p{i}$ is a rule to move the token from every $\p{i}$ vertex in the game, and may take into account the history of the token's path.
The game continues for an infinite duration, giving rise to an infinite sequence of vertices traversed by the token, which is called a \emph{play}.

A vertex with label $c_i$ (in blue) in the game graphs of Fig.~\ref{fig:illustration of assumptions} has \emph{priority} $i$, and the parity winning condition $\Phi$ is satisfied by a play $\rho$ if the maximum priority appearing infinitely often in $\rho$ is even.
We say that a vertex $v$ is \emph{surely winning} for $\pz$ if $\pz$ has a strategy, called the \emph{winning strategy}, such that for every strategy of $\po$, the resulting play starting at $v$ satisfies $\Phi$.
%On the other hand a vertex $v$ is \emph{winning} for $\po$ if $\po$ has a strategy, called the \emph{spoiling strategy}, such that for every strategy of $\pz$, the resulting play starting at $v$ violates $\Phi$.
%If a vertex is not winning for $\pz$ then it is winning for $\po$.
%For example, in Fig.~\ref{fig:illustration of assumptions}.(a), both $p$ and $q$ are winning for $\po$ because $\po$ has a spoiling strategy that moves the token deterministically from $v_0$ to $v_1$ and from $v_1$ to $v_1$ (the only option), written as $v_0\mapsto v_1, v_1\mapsto v_1$, which results in violation of $\Phi$ owing to the ultimately persistent visit to the odd priority $1$.
%It can be shown that every vertex in a parity game graph is winning for either $\pz$ or $\po$.
%
A vertex $v$ is called \emph{cooperatively winning} if there is a joint (possibly coordinated) strategy of $\pz$ and $\po$, called the \emph{joint winning strategy}, such that the resulting play starting at $v$ satisfies $\Phi$.
For example, $p$ in Fig.~\ref{fig:illustration of assumptions}.(a) is a cooperatively winning vertex and the joint winning strategy is $p\mapsto p$ (keep the token in $p$ if it is in $p$), resulting in persistent visits to the even priority $0$.
However, $p$ is not surely winning for $\pz$ because it cannot unilaterally prevent violation of $\Phi$ (by going to $q$ and persistently seeing odd priority $1$).
On the other hand the vertices which are not even cooperatively winning are called \emph{surely losing} (e.g.\ $q$ in Fig.~\ref{fig:illustration of assumptions}.(a)).

\begin{figure}
	\centering
		\begin{subfigure}{.20\textwidth}
		  \centering
		  \begin{tikzpicture}
		  \node[] (duma) at (-0.3,1.4) {\textbf{(a)}};
		  \node[] (dumb) at (2.1,1.4) {\textbf{(b)}};
		  		\node[player1, label=below:{\textcolor{blue}{$c_0$}}] (0) at (0, 0) {$p$};
		  		\node[player0, label=below:{\textcolor{blue}{$c_1$}}] (1) at (\fpeval{\pos}, 0) {$q$};
		  		
		  		\path[->] (0) edge[loop above] () edge node{$e_1$} (1);
		  		\path[->] (1) edge[loop above] ();
		  \end{tikzpicture}
%		  \caption{}
%		  \label{fig:illustration of assumptions}.(a)
		\end{subfigure}
		\begin{subfigure}{.25\textwidth}
		  \centering
		  \begin{tikzpicture}
		  
		  		\node[player0, label=right:{\textcolor{blue}{$c_2$}}] (0) at (0, 0) {$p$};
		  		\node[player1, label=below:{\textcolor{blue}{$c_1$}}] (1) at (-\fpeval{0.75*\pos}, -\pos) {$q$};
				\node[player1, label=below:{\textcolor{blue}{$c_1$}}] (2) at (\fpeval{0.75*\pos}, -\pos) {$r$};
						  		
		  		\path[->] (0) edge[bend left =20] (1) edge[bend right=20] (2);
		  		\path[->] (1) edge[loop left] () edge[bend left =20] node{$e_1$} (0) edge[bend left=20] (2);
				\path[->] (2) 
									edge[loop right] () 
									edge[bend right =20] node[right]{$e_2$} (0) edge[bend left=20] (1);
		  \end{tikzpicture}
%		  \caption{}
%		  \label{fig:illustration of assumptions}.(b)
		\end{subfigure}
		\hspace*{0.05\textwidth}
	\begin{subfigure}{.20\textwidth}
		  \centering
		  \begin{tikzpicture}
		  \node[] (dumc) at (-0.3,1.4) {\textbf{(c)}};
		  \node[] (dumd) at (1.8,1.4) {\textbf{(d)}};
		  		\node[player1, label=below:{\textcolor{blue}{$c_0$}}] (0) at (0, 0) {$p$};
		  		\node[player0, label=below:{\textcolor{blue}{$c_1$}}] (1) at (\fpeval{\pos}, 0) {$q$};
		  		
		  		\path[->] (0) edge[loop above] () edge[bend left = 20] node{$e_1$} (1);
		  		\path[->] (1) edge[bend left = 20] (0);
		  \end{tikzpicture}
%		  \caption{}
%		  \label{fig:illustration of assumptions}.(c)
		\end{subfigure}
		\begin{subfigure}{.25\textwidth}
		  \centering
		  \begin{tikzpicture}
%		  \node[] (dum) at (-1,0.2) {\textbf{(d)}};
		  		  		\node[player1, label=left:{\textcolor{blue}{$c_1$}}] (1) at (0, 0) {$p$};
		  				\node[player1, label=right:{\textcolor{blue}{$c_2$}}] (2) at (\pos, 0) {$q$};
		  				\node[player0, label=below:{\textcolor{blue}{$c_3$}}] (3) at (0,-\pos) {$r$};
		  				\node[player1, label=below:{\textcolor{blue}{$c_4$}}] (4) at (\pos,-\pos) {$s$};
		  				
		  				\path[->] (1) edge[bend left = 20] (2);  		
						\path[->] (2) edge[bend left=20] (1) edge (3) edge[bend left = 20] node{$e_1$} (4);  		
						\path[->] (3) edge (1);
						\path[->] (4) edge[bend left=20] (2);
		  \end{tikzpicture}
%		  \caption{}
%		  \label{fig:illustration of assumptions}.(d)
		\end{subfigure}
%		\caption{Two-player games with the following winning conditions: (a) $\Phi = \square\lozenge v_0$, (b) $\Phi = \square\lozenge v_0$, (c) $\Phi = \lozenge\square v_0$, and (d) $\Phi = C $ with $C = \set{C_i=\set{v_i}}$. }
		\caption{Two-player games with $\po$'s vertices (squares), $\pz$ vertices (circles) and parity winning conditions, where $ c_i $'s denote the priority $ i $ of the vertices. $\p{0}$ wins if the largest priority seen infinitely often is even. }
		\label{fig:illustration of assumptions}
	\end{figure}

We are interested in determining SIM assumptions which convert every cooperatively winning vertex into a sure winning vertex of $\pz$ (sufficiency), which restrict only $\po$'s strategies and that too in a way such that the restrictions can be actually implemented by $\po$ from every vertex (implementability), and lastly which permits every play that satisfies the parity condition $\Phi$ (maximal permissiveness). 
For example, in Fig.~\ref{fig:illustration of assumptions}.(a),  a \aname assumption (that turns $p$ into a surely winning vertex) will be\footnote{We use LTL formulae to simplify notation. Here, \enquote{$\square$} and \enquote{$\lozenge$} denote \enquote{always} and \enquote{eventually}, respectively, and boolean connectives are interpreted in the usual way. See e.g.\ \cite{baier2008principles} for a detailed definition. }  $\assump=\square\lnot e_1$, %\unsure{\AAn{For which winning condition?}}
% \begin{equation}\label{ex:eq:safety assump}	
% \square\lnot e_1,
% \end{equation}
 which is a \emph{safety assumption}.
 
 In Fig.~\ref{fig:illustration of assumptions}.(b), vertices $p,q,r$ are all cooperatively winning (a joint winning strategy is $p\mapsto q, q\mapsto p,  r\mapsto p$) but none of them is sure winning.
	A SIM assumption for fulfilling $\Phi$ will be
	%\begin{equation*}%\label{ex:eq:live group assump}
	$%\[
		\assump=\square\lozenge \set{q,r}\implies \square\lozenge \set{e_1,e_2},
		$
	%\]
	%\end{equation*}
	which is a particular liveness property that we call a \emph{live group assumption}.
	On the other hand, the assumption $\assump'=\square\lozenge e_1 \wedge \square\lozenge e_2$ is sufficient and implementable but \emph{not} maximally permissive, because there is a play $\pi=(pqr)^\omega$ that satisfies $\Phi$ but violates $\assump'$, as $e_1$ is never used along $\pi$.
	
	In Fig.~\ref{fig:illustration of assumptions}.(c), both $p$ and $q$ are cooperatively winning (a joint winning strategy is $p\mapsto p, q\mapsto p$) but none of them is surely winning.
	A SIM assumption for fulfilling $\Phi$ will be $\assump=\lozenge\square\lnot \set{e_1}$, %\unsure{\AAn{What is $ \Phi $?}}
% 	\begin{equation}\label{ex:eq:co-live assump}	
% 		\lozenge\square\lnot \set{e_1},
% 	\end{equation}
	which we call a \emph{co-liveness assumption}.
	On the other hand, the assumption $\assump'=\square\lnot e_1$ is sufficient and implementable but \emph{not} maximally permissive, because there is a play $\pi=pqp^\omega$ that satisfies $\Phi$ but violates $\assump'$, as $e_1$ is taken once along $\pi$.
	
%	\KM{New explanation of Fig.~\ref{fig:illustration of assumptions}.(d):}
%	\new{
	In Fig.~\ref{fig:illustration of assumptions}.(d), all four vertices are cooperatively winning (a joint winning strategy is $p\mapsto q, q\mapsto s, r\mapsto p, s\mapsto q$) but none of them is sure winning.
	Observe that every play will repeatedly see $q$ for every strategy of $\pz$ and $\po$, and a play $\rho$ satisfies $\Phi$ if \emph{either} $r$ appears only finitely many times \emph{or} $s$ appears infinitely many times.
	If we try to enforce only finitely many visits to $r$ by making $(q,r)$ co-live, then we exclude a valid play $ (qrpqs)^{\omega} $.
	On the other hand if we try to enforce infinitely many visits to $s$ by making $\set{(q,s)}$ a live group, then we exclude a valid play $ (qp)^{\omega} $.
	It turns out that in this case, we need a \emph{conditional live group assumption} of the form
% 	\begin{equation*}%\label{ex:eq:cond. live group assump}	
		$\assump=\square\lozenge \set{r}\implies \left( \square\lozenge \set{q} \implies \square\lozenge \set{e_1}\right)$.
% 	\end{equation*}
	%}
	
%	\old{
%	In Fig.~\ref{fig:illustration of assumptions}.(d), all four vertices are cooperatively winning (a joint winning strategy is $v_1\mapsto v_2, v_2\mapsto v_4, v_3\mapsto v_1, v_4\mapsto v_2$) but none of them is sure winning (a spoiling strategy is $v_1\mapsto v_2, v_2\mapsto v_3, v_4\mapsto v_2$).
%	Any assumption that marks some edge co-live, will exclude some cooperatively winning plays. Since at vertices $ v_1,v_3 $ and $ v_4 $, the player has exactly one edge, we do not need any liveness assumptions on them. However, if we mark $ (v_2,v_1) $ live, we exclude $ (v_2v_3v_1v_2v_4)^{\omega} $, and if $ (v_2,v_4) $ is marked live, we exclude $ (v_2v_1)^{\omega} $. Checking all the cases will show that there is no maximally permissive environment assumption using live group fairness and co-live assumptions. A maximally permissive environment assumption for fulfilling $\paritygame(C)$ will be\unsure{shorten the paragraph?}
%	\begin{equation}\label{ex:eq:cond. live group assump}	
%		\square\lozenge \set{v_3}\implies \left( \square\lozenge \set{v_2} \implies \square\lozenge \set{e_1}\right).
%	\end{equation}
%	}
	
	In the remainder of this paper, we show that we can express SIM assumptions for every parity game as a conjunction of safety, co-liveness, and conditional live group assumptions,
	and present efficient symbolic algorithms for computing them. We also apply our algorithm to the well-known 2-client arbiter synthesis problem to show its practical applicability.
	 %\KM{Change other places: conditional -> conditional?}
	%Our algorithm systematically determines all of these conjuncts through efficient symbolic computations over the game graph.
 
%\KM{Change the names of vertices? Later $v_0,v_1,\ldots$ are used to denote the vertices in time $0,1,\ldots$.}
%
%\AKS{I dumped text junks below which should be merged and, by that, shortened. }
%
%
%
% \new{
%If we na\"ively compute assumptions which only require \eqref{eq: assumption as implication} to be winning for $\pz$, then we immediately face two types of ``uninteresting'' but mathematically valid solutions for $\Psi$:
%Firstly, $\Psi$ could be overly restrictive, meaning it may prevent certain environment moves even if they are not harmful.
%For instance, in the game shown in Fig.~\ref{fig:illustration of assumptions}.(c), where $\Phi = \lozenge\square v_0$ (eventually always $v_0$), a valid assumption according to \eqref{eq: assumption as implication} is $\Psi = \bigcirc \square \lnot v_1$ (always avoid $v_1$ from the next step).
%Clearly, both the vertices are winning for $\p{0}$ for the winning condition $\Psi \implies \Phi$, although $\Psi$ restricts all the valid paths which may visit $v_1$ finitely many times.
%Secondly, $\Psi$ could be unimplementable by $\po$, leading to a vacuous satisfaction of the implication in \eqref{eq: assumption as implication}.
%An easy example is $\Psi = \false$, which will ensure that every vertex is winning for $\pz$ for the winning condition $\Psi\implies\Phi$, regardless of what $\Phi$ is.
%Both of these scenarios might prevent any implementation of $\po$ strategy, which is crucial especially when $\po$ models other system components which are also part of the design \cite{emsoft}.
%}
%
%Let us go through our algorithm in an intuitive way.
%A parity winning condition $\Phi$ is specified by labeling every vertex with a unique natural number, where the label of a vertex is called its \emph{priority}.
%The winning condition $\Phi$ is satisfied by a path if the highest priority seen infinitely often is even. 
%Suppose $v$ is a vertex from where the game is only cooperatively winning by $\p{0}$.
%From $v$, there are two possible ways $\po$ may choose to defect, preventing $\pz$ to win, namely (i) $\po$ pushing the game out to a surely losing vertex, or (ii) $\po$ forcing the game to (a) visit a particular odd priority vertex and at the same time (b) depriving visits to any higher even priority vertex.
%We systematically compute assumptions, that restrict $\po$'s choices of edges, preventing these situations to materialize.
%In particular, Cond.~(i) is prevented by assuming that the edges leading to a surely losing vertex is never taken (safety), Cond.~(ii.a) is prevented by assuming that certain edges leading to a high odd priority vertex can be taken only finitely often (called co-liveness), and Cond.~(ii.b) is prevented by assuming that a certain set of edges $H$ leading towards a high even priority vertex is taken infinitely often when certain odd priority vertices are visited infinitely often and when the source vertices of $H$ are visited infinitely often (called transition group fairness).
%\improvement{A better explanation of the algorithm?}
%In Sec.~\ref{sec:motivating example}, we illustrate each of these cases using simple examples, and present the respective maximally permissive and implementable assumptions.
%\KM{define sure winning, cooperative winning etc. somewhere}

% When a parity game graph has $n$ vertices, our algorithm runs in $\mathcal{O}(n^4)$-time, which is independent of the number of priorities.
% \improvement{verify!}
% This is not in conflict with the fact that solving a parity game takes quasipolynomial time and depends on the number of priorities: 
% In our algorithm, we only solve the game cooperatively, which can be done in quadratic time \cite{kupferman}. 
% 
% %\KM{To finish...efficiency, experiments.}
% 
% We implemented our algorithm in the tool called $\tool$, and computed assumptions for the set of parity games in the SYNTCOMP benchmark suite \cite{syntcomp}.
% We empirically showed that our approach is significantly faster than the other approach from the literature, and is successfully able to compute maximally permissive and implementable assumption for every example.




%Automatic synthesis of hardware, software, and cyber-physical systems from a given logical specification is a central problem in computer science \cite{church}.
%These systems are collectively called reactive systems and the synthesis problem is commonly known as reactive synthesis.
%The key features of a reactive system are that they need to \emph{react} to arbitrary environmental inputs and that they are \emph{non-terminating}.
%It has been well-established that the reactive synthesis problem can be reduced, through a chain of reductions involving $\omega$-automata, to the problem of computing winning strategies in games played on directed graphs \cite{buchi_landweber}.

%We consider two-player turn-based zerosum games played on finite graphs and having $\omega$-regular winning conditions.
%We call the two players $\p{0}$ and $\p{1}$.
%Every vertex in the graph is controlled by either of the two players.
%The game is started by initially placing a token in one of the vertices, and then at each turn, the player controlling the token's current location moves the token to one of the successor vertices.
%Given an initial vertex $v$, $\p{0}$ wins the game from $v$ if for every (possibly adversarial) move of $\p{1}$, $\p{0}$ has a strategy such that the infinite path traversed by the token starting from $v$ satisfies the given winning condition.
%Otherwise, $\p{1}$ wins the game from the vertex $v$.

%While a winning strategy for $\p{0}$ for a given initial vertex directly gives us an implementation of the sought reactive system, it is valuable \KM{continue...}

%Graph games form the computational core for the automatic synthesis of hardware, software, and cyber-physical systems from given logical specifications.
%Given a logical specification in some suitable logic like LTL, one can use a chain of reductions going via $\omega$-automata to obtain a two-player game with a parity winning condition \cite{???}.
%If $\vin$ is sure winning (i.e.\ $\vin\in \team{0}\Phi$), then the corresponding winning strategy gives us an implementation of the sought reactive system.
%If $\vin$ is not even cooperative winning (i.e.\ $\vin\notin \team{0,1}\Phi$), then this gives us a certificate of non-existence of a system that can fulfill the specification.
%
%Often the game graph has vertices, called \emph{potentially winning} vertices, which are cooperative winning but not sure winning.
%The set of potentially winning vertices is called the \emph{potentially winning} region, formalized using the set $\team{0,1}\Phi\setminus \team{0}\Phi\neq \emptyset$.
%If $\vin$ is potentially winning, then a reactive system can be constructed only if the environment is assumed to behave in certain manners.

%\subsection{Motivating example}
%\label{sec:motivating example}

%\begin{example}
%\label{ex:illustration of assumptions}
	
	
%	Consider the games shown in Fig.~\ref{fig:illustration of assumptions}.
%	
%	In Fig.~\ref{fig:illustration of assumptions}.(a), vertex $v_0$ is cooperative winning (a joint winning strategy is $v_0\mapsto v_0$), but is not sure winning (a spoiling strategy is $v_0\mapsto v_1$). 
%	A maximally permissive environment assumption will be 
%	\begin{equation}\label{ex:eq:safety assump}	
%	\square\lnot e_1,
%	\end{equation}
%	 which is a \emph{safety} assumption.
%	
%	In Fig.~\ref{fig:illustration of assumptions}.(b), vertices $v_0,v_1,v_2$ are cooperative winning (a joint winning strategy is $v_0\mapsto v_1, v_1\mapsto v_0,  v_2\mapsto v_0$) but none of them is sure winning (a spoiling strategy is $v_1\mapsto v_2, v_2\mapsto v_1$.
%	A maximally permissive environment assumption for fulfilling $\buchigame(\set{v_0})$ will be 
%	\begin{equation}\label{ex:eq:live group assump}		
%		\left(\square\lozenge \set{v_1,v_2}\implies \square\lozenge \set{e_1,e_2}\right),
%	\end{equation}
%	which is a particular type of liveness property that we call a \emph{live group fairness} assumption.
%	A sound but \emph{not} maximally permissive assumption is $\square\lozenge e_1 \wedge \square\lozenge e_2$, because there is a play $(v_0v_1v_2)^\omega$ that is in $\lang(\Phi)$ but violates the assumption ($e_1$ is never used).
%	
%	In Fig.~\ref{fig:illustration of assumptions}.(c), both $v_0,v_1$ are cooperative winning (a joint winning strategy is $v_0\mapsto v_0, v_1\mapsto v_0$) but none of them is sure winning (spoiling strategy is $v_0\mapsto v_1$). 
%	A maximally permissive environment assumption for fulfilling $\cobuchigame(\set{v_0})$ will be
%	\begin{equation}\label{ex:eq:co-live assump}	
%		\lozenge\square\lnot \set{e_1},
%	\end{equation}
%	which we call a \emph{co-live} assumption.
%	A sound but \emph{not} maximally permissive assumption is $\square\lnot e_1$, because there is a play $v_0v_1v_0^\omega$ that is in $\lang(\Phi)$ but violates the assumption ($e_1$ is taken once).
%	
%	In Fig.~\ref{fig:illustration of assumptions}.(d), all three vertices are cooperative winning (a joint winning strategy is $v_1\mapsto v_2, v_2\mapsto v_4, v_3\mapsto v_1, v_4\mapsto v_2$) but none of them is sure winning (a spoiling strategy is $v_1\mapsto v_2, v_2\mapsto v_3, v_4\mapsto v_2$).
%	Any assumption that marks some edge co-live, will exclude some cooperative winning plays. Since at vertices $ v_1,v_3 $ and $ v_4 $, the player has exactly one edge, we do not need any liveness assumptions on them. However, if we mark $ (v_2,v_1) $ live, we exclude $ (v_2v_3v_1v_2v_4)^{\omega} $, and if $ (v_2,v_4) $ is marked live, we exclude $ (v_2v_1)^{\omega} $. Checking all the cases will show that there is no sound and maximally environment assumption using live group fairness and co-live assumptions. A maximally permissive environment assumption for fulfilling $\paritygame(C)$ will be\unsure{shorten the paragraph?}
%	\begin{equation}\label{ex:eq:cond. live group assump}	
%		\square\lozenge \set{v_3}\implies \left( \square\lozenge \set{v_2} \implies \square\lozenge \set{e_1}\right).
%	\end{equation}
%
%	\KM{We need a better one here...}
%\end{example}


==> sections/related_work.tex <==
% !TEX root=main.tex

\section{Related Work}\label{sec:related-work}

%\cite{raman2013towards,hagihara2014minimal} - computes unrealizability core of a given system specification, instead of computing environment assumptions.

%\cite{konighofer2009debugging,bloem2010ratsy} - interactive debugging of unrealizability, not automatic and requires human interaction with the debugger

%\cite{konighofer2010debugging} - weakening system guarantees

%\cite{li2011mining,alur2013counter} - counter-strategy guided mining of assumptions -> some user interaction is needed, the assumptions are LTL properties which is an advantage. no guarantees on maximal permissiveness

%\cite{alur2015pattern,majumdar2020assume} - distributed synthesis using assumptions (maximal permissiveness and automation are important)

%\cite{kim2016directed} - assumption on disturbance values for dynamical system and a given spec
%
%\cite{maoz2019symbolic} - for GR(1), no guarantee on maximal permissiveness
%
%\cite{gaaloul2020mining} - computing assumptions using machine learning based methods - no maximal permissiveness guarantees
%
%\cite{schmelter2017toward,gaaloul2021combining} - evolutionary algorithm based assumption mining, no MP guarantees
%
%\cite{cavezza2020minimal} - minimal set of assumptions for GR(1) specifications - only GR(1)


% Our work is related to cooperative solutions of non-zerosum games and specification-repair in zerosum games.
When considering cooperative solutions of non-zerosum games, related works either fix strategies for both players \cite{ChatterjeeHenzinger_2007,RationalSynthesis_2010} or assume a particularly rational behavior of the environment \cite{BrenguierRaskinSankur_2017}. In contrast, we do not make any assumption on how the environment chooses its strategy. 


% Knowing only the specification for the system player, we compute an assumption which acts as an additional specification for the environment - any environment strategy that fulfills the assumption (in addition to the environment specification) can be used in an actual implementation, allowing for distributed system design resulting in sufficient cooperation.

% Specification-repair is either done by weakening the system guarantees \cite{konighofer2010debugging,raman2013towards,hagihara2014minimal}, or by strengthening the environment assumptions. Our work falls in the second category.
% % 
% Here, some of the earliest work on finding environment assumptions were not fully automatic and they were meant to assist a human designer to debug the specification \cite{konighofer2009debugging,bloem2010ratsy,li2011mining,alur2013counter}.
% Our method, in contrast, is fully automated, which is important for the automated distributed synthesis of reactive systems through repeated generation of assumptions and counter-assumptions \cite{alur2015pattern,majumdar2020assume}.
% % 
% Later on there were many fully automated approaches.
% Some of them use evolutionary optimization algorithms \cite{schmelter2017toward,gaaloul2021combining}, some use machine learning based approaches \cite{gaaloul2020mining}, some use counter-strategy guided algorithms \cite{maoz2019symbolic}, and some of them use a detailed analysis of the underlying game \cite{ChatterjeeHenzingerJobstmann:EnvironmentAssumptionsforSynthesis} like us.
% Unfortunately, all of the aforementioned methods fail to provide maximally permissiveness guarantees.
% A recent work by Cavezza et al.\ \cite{cavezza2020minimal} computes a minimally restrictive set of assumptions but only for GR(1) specifications, which are a strict subclass of the problem considered in our work.
% To the best of our knowledge, we propose the first fully automated algorithm for computing maximally permissive assumptions for general $\omega$-regular games.
% 
% When considering cooperative solutions of non-zerosum games, related works either fix strategies for both players \cite{ChatterjeeHenzinger_2007,RationalSynthesis_2010} or assume a particularly rational behavior of the environment \cite{BrenguierRaskinSankur_2017}. In contrast, we do not make any assumption on how the environment chooses its strategy. Knowing only the specification for the system player, we compute an assumption which acts as an additional specification for the environment - any environment strategy that fulfills the assumption (in addition to the environment specification) can be used in an actual implementation, allowing for distributed system design resulting in sufficient cooperation.

%While our approach is similar to \cite{}, the assumptions we compute are more permissive (for both players) and our algorithm is significantly faster - both theoretically and in practice.  %, allowing maximal freedom in the design of other components within systems of systems. 


%  \begin{remark}
%  A similar notion of sufficient assumptions has also been used by Chatterjee et al.~\cite{ChatterjeeHenzingerJobstmann:EnvironmentAssumptionsforSynthesis}. However, their assumptions are defined for a game with a given initial vertex and a sufficient assumption ensures realiziblity of the specification from this initial vertex only. In our setting, assumptions ensure realizibility from every vertex in the cooperative winning region. This is motivated by controller synthesis problems for cyber-physical systems, where often no initial vertex is specified and the winning region is required to be as large as possible. Moreover, if we consider games with a given initial vertex, then the sufficiency in our setting is different from their setting in two ways:
%   \begin{itemize}
%  \item First, there might be some vertex which is not reachable from the initial vertex, and hence, does not need any restriction on it, but a sufficient assumption in our setting might still put some restrictions on it. However, as that vertex is never reached in a play starting from the initial vertex, the restrictions on that vertex is always vacuously true. Hence, in such cases, the assumptions do not \emph{really} restrict more than they should.
%  \item  Second, there might be some vertex that $\pz$ can avoid visiting and hence, does not need any restriction on it, but again a sufficient assumption in our setting might put some restrictions on it. However, we need such restrictions anyway for permissiveness (i.e., to consider the solutions that visit that vertex) so that it helps in compositional synthesis.
% % In such cases, it helps in solving assumption-based compositional synthesis as it also takes into consideration the plays that visit that vertex. For instance, consider the game in Fig.~\ref{fig:permissive} (right) with initial vertex $v_0$. Here, we do not need any restriction at all, as starting from initial vertex $\pz$ can easily satisfy $\spec_1$ by looping on vertex $v_1$. However, the sufficient assumption $\assump_1$ (and $\assump_0$) made sure that both players \emph{can} satisfy their objective under the assumptions as described in Example~\ref{example:permissive}.
%  \end{itemize}
%  \end{remark}


==> sections/toRemove.tex <==
% !TEX root = main.tex

\smallskip
\section{\color{red}------------To remove---------}

\subsection{\buchi computation}
%We denote by $ Y^i $ the $ i $-th iteration over the fixpoint variable $ Y $. And by $ X_i^j $, we denote $ j $-th iteration of the fixpoint variable $ X $ in the $ i $-th iteration of $ Y $. We know that $ \exists ~k\in \N $ such that $ Y^k=Y^{k+1}=Z^* $, and $\forall ~i\in [0;k], \exists ~l_i\in\N  $ such that $ X_i^{l_i}=X_i^{l_i+1} $. See the table \ref{tab:Buechi} for a visual explanation.
%\bigskip
%\begin{table}\centering
%	\begin{tabular}{cccccccccc}
%		\tikzmark{w}&$ Y^0=V $\tikzmark{x}&&&&&&&&\tikzmark{y}\\
%		&{\color{gray!50}\protect\rotatebox{90}{$\subsetneq$}}&$ X_0^0=\emptyset{\color{gray!50}~\subsetneq}  $&$ X_0^1{\color{gray!50}~\subsetneq}  $&$ \cdots $&&$ X_0^{{\color{red!50}l_0}}\color{gray!50}{~=} $&$ X_0^{l_0+1}  $&&\\
%		&$ Y^1 $&&&&&&&&\\
%		&{\color{gray!50}\protect\rotatebox{90}{$\subsetneq$}}&$ X_1^0=\emptyset{\color{gray!50}~\subsetneq}  $&$ X_1^1{\color{gray!50}~\subsetneq}  $&$ \cdots $&&&&$ X_1^{{\color{red!50}l_1}}\color{gray!50}{~=} $&$ X_1^{l_1+1} $\\
%		&$ Y^2 $&&&&&&&&\\
%		&{\color{gray!50}\protect\rotatebox{90}{$\subsetneq$}}&$ X_2^0=\emptyset{\color{gray!50}~\subsetneq}  $&$ X_2^1{\color{gray!50}~\subsetneq}  $&$ \cdots $&&&$ X_2^{{\color{red!50}l_2}}{\color{gray!50}{~=}} $&$ X_2^{l_2+1} $&\\
%		&$ \vdots $&&&&&&&&\\
%		&$ Y^{\color{red!50}k} $&&&&&&&&\\
%		&{\color{gray!50}\protect\rotatebox{90}{$=$}}&$ X_k^0=\emptyset{\color{gray!50}~\subsetneq}  $&$ X_k^1{\color{gray!50}~\subsetneq}  $&$ \cdots $&$ X_k^{{\color{red!50}l_k}}\color{gray!50}{~=} $&$ X_k^{l_k+1} $&&&\\
%		\tikzmark{z}&$ Y^{k+1}=Z^* $&&&&&&&&\\
%	\end{tabular}
%	\begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt]
%		\draw [->, thick] ([yshift=\baselineskip]{pic cs:x}) -- ([yshift=\baselineskip]{pic cs:y})node[midway,above] {Iterations over $ X $ with fixed $ Y^i $};
%		\draw [->, thick] ({pic cs:w}) -- ({pic cs:z})node[midway,left] {\protect\rotatebox{90}{Iterations over $ Y $}};
%	\end{tikzpicture}
%	\caption{\label{tab:Buechi}B\"uchi fixpoint computation}
%\end{table}


\subsection{\cobuchi computation}


We denote by $ X^i $ the $ i $-th iteration over the fixpoint variable $ X $. And by $ Y_i^j $, we denote $ j $-th iteration of the fixpoint variable $ Y $ in the $ i $-th iteration of $ X $. We know that $ \exists ~k\in \N $ such that $ X^k=X^{k+1}=Z^* $, and $\forall ~i\in [0;k], \exists ~l_i\in\N  $ such that $ Y_i^{l_i}=Y_i^{l_i+1} $. See the table \ref{tab:coBuechi} for a visual explanation.

\begin{table}\centering
	\begin{tabular}{cccccccccc}
		\tikzmark{a}&$ X^0=\emptyset $\tikzmark{b}&&&&&&&&\tikzmark{c}\\
		&{\color{gray!50}\protect\rotatebox{90}{$\supsetneq$}}&$ Y_0^0=V{\color{gray!50}~\supsetneq}  $&$ Y_0^1{\color{gray!50}~\supsetneq}  $&$ \cdots $&&$ Y_0^{{\color{red!50}l_0}}\color{gray!50}{~=} $&$ Y_0^{l_0+1}  $&&\\
		&$ X^1 $&&&&&&&&\\
		&{\color{gray!50}\protect\rotatebox{90}{$\supsetneq$}}&$ Y_1^0=V{\color{gray!50}~\supsetneq}  $&$ Y_1^1{\color{gray!50}~\supsetneq}  $&$ \cdots $&&&&$ Y_1^{{\color{red!50}l_1}}\color{gray!50}{~=} $&$ Y_1^{l_1+1} $\\
		&$ X^2 $&&&&&&&&\\
		&{\color{gray!50}\protect\rotatebox{90}{$\supsetneq$}}&$ Y_2^0=V{\color{gray!50}~\supsetneq}  $&$ Y_2^1{\color{gray!50}~\supsetneq}  $&$ \cdots $&&&$ Y_2^{{\color{red!50}l_2}}{\color{gray!50}{~=}} $&$ Y_2^{l_2+1} $&\\
		&$ \vdots $&&&&&&&&\\
		&$ X^{\color{red!50}k} $&&&&&&&&\\
		&{\color{gray!50}\protect\rotatebox{90}{$=$}}&$ Y_k^0=V{\color{gray!50}~\supsetneq}  $&$ Y_k^1{\color{gray!50}~\supsetneq}  $&$ \cdots $&$ Y_k^{{\color{red!50}l_k}}\color{gray!50}{~=} $&$ Y_k^{l_k+1} $&&&\\
		\tikzmark{d}&$ X^{k+1}=Z^* $&&&&&&&&\\
	\end{tabular}
	\begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt]
		\draw [->, thick] ([yshift=\baselineskip]{pic cs:b}) -- ([yshift=\baselineskip]{pic cs:c})node[midway,above] {Iterations over $ Y $ with fixed $ X^i $};
		\draw [->, thick] ({pic cs:a}) -- ({pic cs:d})node[midway,left] {\protect\rotatebox{90}{Iterations over $ X $}};
	\end{tikzpicture}
	\caption{\label{tab:coBuechi}\cobuchi fixpoint computation}
\end{table}

\subsection{iterative algorithms}

\begin{algorithm}
	\caption{FindB\"uchiAssumptions(\game)}
	\label{alg:find buchi assumptions}
	\begin{algorithmic}[1]
		\Require $ \game=\tup{V=(V^0,V^1),E,C:V\rightarrow \{1,2\}, \Phi = \square\lozenge C_2} $
		\Ensure $\assump$
		\State $ S=\emptyset, \livegroup=\emptyset $
		\State $W^*\gets B\ddot{u}chi^{0,1}(C_2)$
		\State $ S\gets E \cap (W^* \times V\backslash W^*)$ \Comment{All edges leaving $ W^* $}
		\State $ G\gets G|_{W^*} $
		\State $W^0 \gets C_2\cap W^*$, $W^1\gets \attrz{}{W^0}$
		\State $i\gets 1$
		\While{$W^*\neq W^i$}
		\State $Z^i \gets \pre{}{W^{i}}$ \Comment{$ Z^i\backslash W^i \subseteq V^1$}
		\State $E^{i}\gets \Set{(v,v') \in E \mid v\in Z^i\backslash W^i \, \wedge\, v'\in W^{i}}$ \Comment{Edges from $ Z^i $ to $ W^i $}
		\State $\livegroup \gets \livegroup \cup \Set{E^{i}}$
		\State $ W^{i+1}\gets \attrz{}{W^i\cup Z^i} $
		\State $ i\gets i+1 $
		\EndWhile
		\State \Return $\assump = \assumpsafe(S)\cap \assumpgrlive(\livegroup) $
	\end{algorithmic}
\end{algorithm}

Here we use a standard procedure $ B\ddot{u}chi^{0,1} $ to compute the co-operative winning region $ \team{0,1} \Phi $.
We show that $ \assump $ computed by Alg.~\ref{alg:find buchi assumptions} gives a maximally permissive sound assumption for B\"uchi.


\begin{lemma}\label{lem:buchi termination}
	Alg. \ref{alg:find buchi assumptions} terminates, with $  W^1\subsetneq W^2\subsetneq\cdots \subsetneq W^p=W^*,  $
	where $ p\leq |V| $.
\end{lemma}
\begin{proof}
	By the monotonicity of $ \textsf{attr}^0 $, for all $ i\geq 1, W^i\subseteq W^{i+1} $. Note that if for some $ i $, $ W^i=W^{i+1} $, then for all $ j>i, W^j=W^i $, since $ Z^j=\emptyset $, and hence $ W^j=\attrz{}{W^{j-1}}=\attrz{}{W^{i}}=W^i $.
	
	\begin{claim}\label{claim:buchi algo terminates with whole winning set}
		If for some $ i, W^i=W^{i+1} $, then $ W^i=W^* $. 
	\end{claim}
	\begin{proof}[Claim \ref{claim:buchi algo terminates with whole winning set}]
		Suppose not, i.e. let $ v\in W^*\backslash W^i $. Since $ v\in B\ddot{u}chi^{0,1}(C_2) $, then there is a path from $ v$ to $ W^0 $. Consider the path without a cycle $ \rho $ with maximum number of vertices $ k $ in $ V^1 $, before seeing a vertex in $ W^i $. Note that $ k>0 $, else $ v\in W^{i}=\attrz{}{W^i\cup Z^i} $. But then $ Z^{i}\not=\emptyset $, which would a contradiction to the fact that $ W^i\not=W^{i+1} $.\tqed
	\end{proof}
	
	Hence, in every iteration of the while loop, at least one vertex is added to $ W^i $, untill no more can be added, in which case $ W^i=W^* $. Hence, Alg. \ref{alg:find buchi assumptions} terminates. Since at most $ |V| $ many vertices can be added, $ p\leq |V| $.\qed
\end{proof}


\begin{lemma}\label{lemma:buchi sound assumption}
	$ \assump $ returned by Alg. \ref{alg:find buchi assumptions} is a sound environment assumption.
\end{lemma}
\begin{proof}
	We observe that $ Z^i\backslash W^i\subseteq V^1 $, i.e. every vertex in $ Z^i $ is either a $ \po $ vertex or it is already in $ W^i $: since if $ v\in Z^i\cap V^0$, it would already be in $ \attrz{}{W^{i-1}\cup Z^{i-1}} $. Hence, every $ \pz $ vertex is added to some $ W^i $ in the $ \textsf{attr}^0 $ computation step in the while loop.
	
	Hence, $ V^0\cap W^* $ can be partitioned into sets $ V_1, V_2\ldots, V_p $, where $ V_i= (W^i\backslash W^{i-1})\cap V^0 $. 
	
	Consider the strategy $ \pi^0 $ for $ \pz $: at a vertex $ v\in V_i $, plays the $ \textsf{attr}^0 $ strategy to reach $ W^{i-1}\cup Z^{i-1} $, and for other vertices, plays arbitrarily.
	
	Let $ \rho=v_0v_1\ldots $ be a $ \pi^0 $-play such that $ \rho\in\assump $. Since $ \rho\in\assumpsafe(S) $, $ v_i\in W^* $ for all $ i $. Now, suppose $ \rho \not\in \Phi $. Then $ i\in [1,p] $, such that $ inf(\rho)\cap W^i\not= \emptyset $ but $ inf(\rho)\cap W^j= \emptyset,~ \forall j<i $.
	
	By the definition of $ \pi^0 $, every time $ \rho $ visits $ W^i $, it also eventually visits $ W^{i-1}\cup Z^{i-1} $. If $ \rho $ visits $ W^{i-1} $ infintely often, it contradicts with our assumption that $ inf(\rho)\cap W^{i-1} =\emptyset$. But if $ Z^{i-1} $ is visited infinitely often, by the definition of $ \livegroup $, an edge $ (v,v')\in E^{i-1} $ is taken infinitely often, where $ v'\in W^{i-1} $, which contradicts with our assumption again.
	
	Hence, $ \rho\in\Phi $. \qed
\end{proof}

\begin{lemma}\label{lem:buchi max permissive}
	$ \assump $ returned by Alg. \ref{alg:find buchi assumptions} is maximally permissive.
\end{lemma}

\begin{proof}
	Let $ \rho\in \Phi $. Suppose that $ \rho\not\in\assump $. 
	
	Case 1: If $ \rho\not\in\assumpsafe(S) $. Then some edge $ (v,v')\in S $ is taken in $ \rho $. Then after reaching $ v' $, $ \rho $ still satisfies the B\"uchi objective. Hence, $ v'\in W^* $, but then $ (v,v')\not\in S $, which is a contradiction.
	
	Case 2: If $ \rho\not\in\assumpgrlive(\livegroup) $. Then $ \exists E^i\in H^l, $ such that $ \rho $ visits $ src(E^i)=Z^i\backslash W^i $ infinitely often, but no edge in $ E^i $ is taken infinitely often, i.e. play stays in $ W^{i+1}\backslash W^i $ or goes to $ W^{j}\backslash W^i $ for some $ j>i+1 $. In the first case, since $ C_2\cap W^*\subseteq W^i $, $ \rho\not\in\Phi $, which would be a contradiction. On the other hand, in the second case, after going to $ W^j $, $ \rho $ has an edge going from some $ v\in W^*\backslash W^{j-1} $ to some $ v'\in W^i $ (else $ C_2 $ can not be reached). But then $ v $ would be added to $ W^{i+1} $, which contradicts to the fact that $ j>i+1 $.
	
	In either case, we get a contradiction, so $ \rho\in\assump$. 
\end{proof}












\add{Explain with pictures/examples}
\begin{algorithm}
	\caption{FindCo-B\"uchiAssumptions(\game)}
	\label{alg:find cobuchi assumptions}
	\begin{algorithmic}[1]
		\Require $ \game=\tup{V=(V^0,V^1),E,C:V\rightarrow \{0,1\}, \Phi = \lozenge\square \neg C_1} $
		\Ensure $\assump$
		\State $ S\gets\emptyset, D\gets\emptyset, \livegroup\gets\emptyset $
		\State $W^*\gets Co\text{-}B\ddot{u}chi^{0,1}(C_1)$ 
		\State $ S\gets E \cap (W^* \times V\backslash W^*)$ \Comment{All edges leaving $ W^* $}
		\State $ G\gets G|_{W^*} $
		\State $ G'\gets G|_{V\setminus C_1} $
		\State $ \Wno \gets B\ddot{u}chi^{0,1}_{G'}(C_0) $
		\State $ D\gets \Set{(v,v')\in E\mid v\in \Wno\wedge v'\in W^*\setminus \Wno} $
		\State $ \Phi\gets \square \lozenge \Wno $
		\State $ H^l\gets FindB\ddot{u}chiAssumptions(\game)  $\label{step:call Buchi algo}
		\State \Return $\assump = \assumpsafe(S)\cap \assumpgrlive(\livegroup)\cap \assumpdep(D) $
	\end{algorithmic}
\end{algorithm}

Here, we again use standard procedures $ Co$-$B\ddot{u}chi $ and $ B\ddot{u}chi $, and the subscript mentions the game in considration. Step \ref{step:call Buchi algo} calls Algo. \ref{alg:find buchi assumptions} to find live transition groups after the update in the objective.

\begin{lemma}\label{lemma:cobuchi sound assumption}
	$ \assump $ returned by Alg. \ref{alg:find cobuchi assumptions} is a sound environment assumption.
\end{lemma}

\begin{proof}
	Consider the strategy $ \pi^0 $ for $ \pz $: if the vertex is in $ \Wno $, then play the $ B\ddot{u}chi^{0,1}_{G'}(C_0) $ strategy, if the vertex is in $ W^*\setminus \Wno $, then play the strategy as in the Lemma \ref{lemma:buchi sound assumption}, else play arbitrarily.
	
	Let $ \rho=v_0v_1\ldots $ be a $ \pi^0 $-play such that $ \rho\in\assump $ and $ v_0\in W^* $. Suppose that $ \rho\not\in\Phi $, then $ inf(\rho)\cap C_1\not=\emptyset $. Note that $ \forall i. ~ v_i\in W^* $, since $ \rho\in\assumpsafe(S) $.
	
	Case 1: $ inf(\rho)\subseteq\Wno $. Then since $ C_1\cap \Wno=\emptyset $, the play eventually visits only $ C_0 $, i.e. $ \rho\in\Phi $, which is a contradition.
	
	Case 2: $ \inf(\rho)\cap (W^*\setminus \Wno)\not=\emptyset $. Then by the correctness of Alg. \ref{alg:find buchi assumptions}, it follows that $ \Wno $ is visited infinitely often. But then visiting $ W^*\setminus\Wno $ requires taking edges in $ D $ infinitely often. Hence, $ \rho\not\in\assumpdep(D) $, which is a contradiction again.
	
	In either case, we get a contradiction. Hence, $ \rho\in\Phi $.
\end{proof}


\begin{lemma}\label{lem:cobuchi max permissive}
	$ \assump $ returned by Alg. \ref{alg:find cobuchi assumptions} is maximally permissive.
\end{lemma}

\begin{proof}
	Let $ \rho\in \Phi $. Suppose that $ \rho\not\in\assump $. 
	
	Case 1: If $ \rho\not\in\assumpsafe(S) $. This gives a contradiction as in the proof of Lemma \ref{lem:buchi max permissive}.
	
	
	Case 2: If $ \rho\not\in\assumpgrlive(\livegroup) $. Note that since $ \rho\in\Phi $, $ C_1 $ is visited only finitely often. Then consider the suffix $ \rho' $ of $ \rho $ such that no vertex in $ C_1 $ appears in $ \rho' $. $ \rho $ eventually stays in $ \Wno $: if some $ v\in (W^*\setminus\Wno)\cap C_0  $ appears in $ \rho' $, then $ v $ would have been in $ \Wno $, since there is play  (in particular, $ \rho' $)  satisfying $ \Phi $. \add{maybe needs a lemma?}
	
	
	Then by the arguments as in the proof of Lemma \ref{lem:buchi max permissive}, $ \rho\not\in\assumpgrlive(\livegroup) $ implies that $ \rho $ does not saturate in $ \Wno $ eventually, which is a contradiction.
	
	
	Case 3: If $ \rho\not\in\assumpdep(D) $. Then some edge $ (u,v)\in D $ is taken infinitely often. Then again as in previous case, $ C_1 $ appears only finitely often, so $ v\in(W^*\setminus\Wno)\cap C_0  $. But then again $ v $ would have been in $ \Wno $, i.e. $ (u,v)\not\in D $, resulting in a contradiction.
	
	
	In any case, we get a contradiction, so $ \rho\in\assump $.
\end{proof}









\begin{algorithm}
	\caption{FindLiveTransitionGroups}
	\label{alg:find live tr groups}
	\begin{algorithmic}[1]
		\Require $ \game=\tup{V=(V^0,V^1),E,C:V\rightarrow \{1,2\}, \Phi = \square\lozenge C_2} $
		\Ensure $\livegroup$
		\State $W^*\gets\team{0,1}\square\lozenge B$
		\State $W^0 \gets B\cap W^*$, $W^1\gets \team{0}\lozenge W^0$
		\State $\livegroup = \emptyset$
		\State Compute $\assumpsafe$ (refer to \cite{chatterjee2008environment}) %\Comment{Takes care of the fact that}
		\State $i\gets 1$
		\While{$W^*\neq W^i$}
		\State $i\gets i+1$
		\State $Z^i \gets \team{0,1}\bigcirc W^{i-1}$ \Comment{$Z\subseteq \vertexo$}
		\State $E^{Z,i}\gets \Set{(v,v') \mid v\in Z^i \, \wedge\, v'\in W^{i-1} \cap \edge(v)}$
		\State $\livegroup \gets \livegroup \cup \Set{E^{Z,i}}$
		\State Compute $\assumpgrlive$ for $\livegroup$
		\State $\assump \gets \assumpsafe\cap \assumpgrlive$
		\State $W^i\gets \team{0}(\assump \implies\lozenge W^0)$ \Comment{\KM{Equivalently, $W^i\gets \team{0}W^*\mathcal{U} (W^{i-1}\cup \src(\livegroup))$?}} %\Comment{Equivalently, $W^i\gets \team{0}(\assump\implies\lozenge W^0)$}
		\EndWhile
		\State \Return $\livegroup$
	\end{algorithmic}
\end{algorithm}


\begin{lemma}\label{lem:monotonic W^i}
	The sequence $W^0,W^1,\ldots,W^p=W^*$ computed by Alg.~\ref{alg:find buchi assumptions} is monotonically increasing with respect to set inclusion ``$\subseteq$.''
\end{lemma}

\begin{proof}
	Follows from the monotonicity of $ \mathsf{attr}^0 $.\tqed
\end{proof}

Suppose $W^0,W^1,\ldots,W^p=W^*$ be the sequence of $W^i$-s computed by Alg.~\ref{alg:find live tr groups}.
We introduce a ranking function $\rankfun\colon W^*\to [0;p]$ that assigns a rank to the vertices in $W^*$ as follows:
if $v\in W^m\setminus W^{m-1}$ for some $m\in [0;p]$, then $\rankfun(v)=m$.
Since the sequence $W^0,W^1,\ldots,W^p$ is monotonic (see Lem.~\ref{lem:monotonic W^i}), hence the function $\rankfun$ is well-defined.

A set of vertices $T$ is called a \emph{trap} (for $\pz$) if $T = \team{1}\square T$.
Intuitively, a trap is a part of the game graph where $\po$ can confine the game forever.

\begin{lemma}\label{lem:trap}
	For every $i\in [1;p]$, $\vertex\setminus W^i$ is a trap.
\end{lemma}

\begin{proof}
	Had the claim not been true, then there would be a vertex $v\in \vertex\setminus W^i$ such that $v\in \team{0}\lozenge W^i$ (from determinacy of two-player games with $\omega$-regular objectives).
	This would imply that $v$ is itself in $W^i$, which contradicts our assumption.
\end{proof}

\begin{lemma}\label{lem:role of live tr group}
	Every infinite play $\pi$ starting from a vertex $v\in \vertex\setminus W^i$ with $i\in [1;p]$ satisfies \emph{either} of the following:
	\begin{enumerate}[(A)]
		\item $\pi$ remains forever confined in, i.e.\ $\pi\in \square\vertex\setminus W^i$. \label{lem:role of live tr group:opt a}
		\item $\po$ eventually picks an edge from the set $E^{Z,i+1}$, i.e.\ there exists $(r,r')\in E^{Z,i+1}$ and there exists $k\in \mathbb{N}$ such that $\pi(k) = r$ and $\pi(k+1)=r'$.\label{lem:role of live tr group:opt b}
	\end{enumerate}
\end{lemma}

\begin{proof}
	Since $\vertex\setminus W^i$ is a trap (see Lem.~\ref{lem:trap}), hence $\po$ has a strategy such that the play remains confined inside $\vertex\setminus W^i$ forever, which means that \eqref{lem:role of live tr group:opt a} can be true.
	If \eqref{lem:role of live tr group:opt a} is not true, then the play eventually has to cross an edge from the set $E^{Z,i+1}$, which is the set of all possible edges that can be taken to reach $W^i$ in a cooperative manner.
	This accounts for \eqref{lem:role of live tr group:opt b}.
\end{proof}

\begin{theorem}
	Alg.~\ref{alg:find live tr groups} is sound and the computed live transition groups induce a maximally permissive fairness assumption on the environment.
\end{theorem}

\begin{proof}
	Soundness means that the $\livegroup$ obtained indeed induces a sound assumption.
	This follows from the fact that $\assumpsafe$ takes care of the fact that the game does not leave $W^*$ after reaching $B\cap W^*$, and from the fact that $B\cap W^*$ can be reached from every vertex in $W^*\setminus B$ (ensured by the guard condition of the while loop).
	\KM{Lem.~\ref{lem:monotonic W^i} will be needed here if we want to do the proof more rigorously.}
	
	For maximal permissiveness, we need to show that if there is an infinite play $\pi$ that satisfies $\spec$, then $\pi$ is allowed by $\assumpsafe$ and $\assumpgrlive$ induced by $\livegroup$, i.e.\
	\begin{equation}
		\pi\in\spec \implies \pi\in \assumpsafe \cap \assumpgrlive.
	\end{equation}
	The fact that $\pi\in\spec\implies\pi\in \assumpsafe$ follows from \cite[Thm.~5]{chatterjee2008environment}.
	\KM{Check!}
	\new{	
		So we only focus on proving $\pi\in \spec\implies \pi\in\assumpgrlive$.
		
		Suppose, the claim is not true, i.e.\ there is a play $\pi$ that satisfies $\spec$, and yet violates $\assumpgrlive$ by visiting $\src(E^{Z,i+1})$ infinitely often but taking the edges in $E^{Z,i+1}$ only finitely often for some $i\in [1;p]$.
		Let $k\in \mathbb{N}$ be the time instant when an edge from $E^{Z,i+1}$ was taken for the last time.
		There is a $k'>k$ when some vertex $v\in\src(E^{Z,i+1})$ is visited, since $\src(E^{Z,i+1})$ is visited infinitely often according to our asumption.
		The vertex $v$ belongs to $\vertex\setminus Z^i$ as per our construction.
		The suffix $\pi|_{[k',\infty)}$ of the play $\pi$, which is itself an infinite play starting at $v$, does not satisfy \eqref{lem:role of live tr group:opt b} in Lem.~\ref{lem:role of live tr group}.
		So $\pi|_{[k',\infty)}$ must satisfy \eqref{lem:role of live tr group:opt a} in Lem.~\ref{lem:role of live tr group}.
		Hence, from $k'$ time onward, $\pi$ will never visit $W^0=B\cap W^*$, which implies that $\pi\notin \spec$, contradicting our assumption in the first place.}
\end{proof}

